TraveLER: A Modular Multi-LMM Agent Framework for Video Question-Answering

Recently, image-based Large Multimodal Models (LMMs) have made significant progress in video question-answering (VideoQA) using a frame-wise approach by leveraging large-scale pretraining in a zero-shot manner. Nevertheless, these models need to be capable of finding relevant information, extracting it, and answering the question simultaneously. Currently, existing methods perform all of these steps in a single pass without being able to adapt if insufficient or incorrect information is collected. To overcome this, we introduce a modular multi-LMM agent framework based on several agents with different roles, instructed by a Planner agent that updates its instructions using shared feedback from the other agents. Specifically, we propose TraveLER, a method that can create a plan to "Traverse" through the video, ask questions about individual frames to "Locate" and store key information, and then "Evaluate" if there is enough information to answer the question. Finally, if there is not enough information, our method is able to "Replan" based on its collected knowledge. Through extensive experiments, we find that the proposed TraveLER approach improves performance on several VideoQA benchmarks without the need to fine-tune on specific datasets. Our code is available at https://github.com/traveler-framework/TraveLER.

==> sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

Our {\smodel} framework has demonstrated significant potential in utilizing a multi-agent LMM image-based approach for video QA. We introduce an agent-based framework that travels along the video, collecting relevant information from key frames through interactive question-asking until there is sufficient information to answer the question. Our method stands out by creating a plan to ``traverse'' through the video, asking questions about individual frames to ``locate'' and store key information, and then ``evaluate'' if there is enough information to answer the question. Finally, if there is not enough information, our model is able to ``replan'' according to its collected knowledge. The substantial improvements observed on video question-answering benchmarks, such as NExT-QA, STAR, and Perception Test, without the need to fine-tune on specific datasets highlight the effectiveness of our approach across a diverse set of datasets. Our research encourages future work in leveraging large models to develop more robust and modular approaches for video understanding.

==> tables/ablation_component.tex <==
    \begin{tabular*}{lc}
        \toprule
        Component & Accuracy\\
        \midrule
        Planner & 58.1 \\
        Retriever & 56.9 \\
        Extractor & 58.2 \\
        Summarizer & 57.2 \\
        \bottomrule
    \end{tabular*}

==> tables/agent_ablations.tex <==
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\begin{table*}[tb!]
    \vspace{-0.2em}
    \caption{\textbf{Agent Ablations.} We report ablations on each component of our framework: (a) Planner (b) Retreiver (c) Extractor (d) Evaluator}
    \centering
    %\begin{subtable}[t]{.3\linewidth}
    \begin{subtable}[t]{.3\linewidth}
	\tablestyle{5pt}{1.25}
        \centering
        \caption{{Replacing Diff. LLMs}}
        \label{tab:agents_llm}
        
        \begin{tabular}{lccc}
            \toprule
            Planner & Accuracy \\
            \midrule
            No Change & 65.8
            Removal & 63.5 \\
            Fixed Plan &  & 63.5\\
            \bottomrule
        \end{tabular}
        
    \end{subtable}
    \begin{subtable}[t]{.25\linewidth}
	\tablestyle{5pt}{1.25}
        \centering
        \caption{{Replacing Diff. LMMs}}
        \label{tab:agents_lmm}

         \begin{tabular}{lccc}
            \toprule
            Planner & Accuracy \\
            \midrule
            No Change & 65.8
            Removal & 62.3 \\
            \bottomrule
        \end{tabular}

        
    \end{subtable}
    %\hfill
    \hspace{18pt}
    \begin{subtable}[t]{0.15\linewidth}
        \tablestyle{3pt}{1.25}
        \centering
	    \caption{{\# of Frames}}
        \label{tab:retriever}

        \begin{tabular}{lccc}
            \toprule
            Extractor & Accuracy \\
            \midrule
            No Change & 65.8
            Caption Only & 60.1 \\
            \bottomrule
        \end{tabular}

 
    \end{subtable}
    \hspace{8pt}
    \begin{subtable}[t]{0.2\linewidth}
	\tablestyle{3pt}{1.25}
	% \scriptsize
        \centering
        \caption{{\# of Questions}}
        \label{tab:questions}

        \begin{tabular}{lccc}
            \toprule
            Evaluator & Accuracy \\
            \midrule
            No Change & 65.8
            Removal & 62.2 \\
            \bottomrule
        \end{tabular}

    \end{subtable}
    \vspace{-10pt}
    \label{tab:ablations}
\end{table*}

\renewcommand{\thefootnote}{\arabic{footnote}}


==> tables/star_and_perception.tex <==
\tabcolsep=0.11cm
\begin{table*}[t]
    \begin{minipage}[c]{0.6\textwidth}
        \caption{ZS results on STAR.}
        \label{tab:star}
        \centering
        \begin{tabular}{lccccc}
            \toprule
            Model & Int. & Seq.& Pre. & Fea. & Avg. \\
            \midrule
            \rowcolor{gray!20} SeViLA & 48.3 & 45.0 & 44.4 & 40.8 & 44.6 \\
            \midrule
            Flamingo-9B & - & - & - & - & 41.8 \\
            InternVideo & 43.8 & 43.2 & 42.3 & 37.4 & 41.6\\    
            BLIP-2\textsuperscript{voting} & 41.8 & 39.7 & 40.2 & 39.5 & 40.3\\
            BLIP-2\textsuperscript{concat} & \textbf{45.5} & 41.8 & 41.8 & 40.0 & 42.2\\
            \rowcolor{lavendermist} TraveLER (ours) & 43.3 & \textbf{45.9} & \textbf{45.8} & \textbf{42.8} & \textbf{44.9} \gcol{+2.7} \\
        \bottomrule
    \end{tabular}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.4\textwidth}
        \caption{ZS results on Perception Test.}
        \label{tab:perception}
        \centering
        \begin{tabular}{lc}
            \toprule
            Model & Test Accuracy\\
            \midrule
            \rowcolor{gray!20} SeViLA & 46.2 \\
            \rowcolor{gray!20} MC-ViT-B & 47.0  \\
            \rowcolor{gray!20} MC-ViT-L & 48.1 \\
            \midrule
            Flamingo-3B & 43.6 \\
            LongViViT & 45.7\\
            \rowcolor{lavendermist} TraveLER (ours) & \textbf{50.2} \gcol{+4.5} \\
            \bottomrule
        \end{tabular}
    \end{minipage}
\end{table*}
